3DGS-Calib: 3D Gaussian Splatting for Multimodal SpatioTemporal Calibration

Reliable multimodal sensor fusion algorithms require accurate spatiotemporal calibration. Recently, targetless calibration techniques based on implicit neural representations have proven to provide precise and robust results. Nevertheless, such methods are inherently slow to train given the high computational overhead caused by the large number of sampled points required for volume rendering. With the recent introduction of 3D Gaussian Splatting as a faster alternative to implicit representation methods, we propose to leverage this new rendering approach to achieve faster multi-sensor calibration. We introduce 3DGS-Calib, a new calibration method that relies on the speed and rendering accuracy of 3D Gaussian Splatting to achieve multimodal spatiotemporal calibration that is accurate, robust, and with a substantial speed-up compared to methods relying on implicit neural representations. We demonstrate the superiority of our proposal with experimental results on sequences from KITTI-360, a widely used driving dataset.

==> figures/downsampling.tex <==
\begin{figure}[!htbp]
\centering
\scriptsize
\setlength{\tabcolsep}{0.002\linewidth}
    \begin{tabular}{c}
        \includegraphics[width=0.9\linewidth]{figures/full_pcd.png}\\
        \includegraphics[width=0.9\linewidth]{figures/downsample10_pcd.png}
    \end{tabular}
\caption{\textbf{Accumulated LiDAR point cloud --} The accumulated point cloud from the LiDAR scans (top) and the downsampled version with voxel size 10 cm (bottom). \LR{for me, this figure doesnt have any interest, I would remove it, or make it considerably smaller in any case. If you consider the figure and the text, half a page of your paper consists on a pointcloud downsampling...}}
\label{fig:downsample}
\end{figure}

==> tables/loss_ablation.tex <==
\begin{table}[b]
\centering
\scriptsize
\caption{\label{tab:loss_ablation} Ablation study on losses with spatiotemporal calibration (\textbf{best} and \underline{second best}).}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{} l l ll l ll l l @{}}
\toprule
 & Translation error & Rotation error & Temporal error \\
Loss & (cm) & (°) &  (ms) \\
\hline
$L_C$ + $L_D$ & $7.4\pm1.2$ & $0.31\pm0.06$ & $4.4\pm1.0$ \\
$L_C$ + $L_D$ + SSIM & $\underline{6.9\pm1.3}$ & $\underline{0.30\pm0.04}$ & $\bm{1.9\pm0.6}$ \\
$L_C$ + $L_D$ + DS & $14.4\pm2.1$ & $0.31\pm0.14$ & $4.4\pm0.8$ \\
$L_C$ + $L_D$ + SSIM+DS & $\bm{6.8\pm1.0}$ & $\bm{0.28\pm0.06}$ & $\underline{2.8\pm0.6}$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/opti_ablation.tex <==
\begin{table*}[hbt!]
\centering
\scriptsize
\caption{\label{tab:opti_ablation} Ablation study on optimized parameters.}

\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{} l lll l lll l lll @{}}
\toprule
& \multicolumn{3}{c}{Front-Right Camera} && \multicolumn{3}{c}{LiDAR} \\
\cmidrule{2-4} \cmidrule{6-8}
Optimized parameters & Translation error (cm) & Rotation error (°) & Temporal error (ms) && Translation error (cm) & Rotation error (°) & Temporal error (ms) \\
\hline
Only spatial & $103.0\pm1.0$ & $1.03\pm0.03$ & -- && $104.8\pm2.3$ & $0.35\pm0.07$ & --\\
Only temporal & -- & -- & $89.6\pm0.2$ && -- & -- & $100.9\pm0.8$\\
Spatial \& temporal & $1.9\pm0.6$ & $0.08\pm0.01$ & $1.2\pm0.3$ && $11.5\pm2.1$ & $0.44\pm0.07$ & $10.1\pm1.3$\\
\bottomrule
\end{tabular}
\end{table*}

==> tables/opti_pose_ablation.tex <==
\begin{table*}[hbt!]
\centering
\scriptsize
\caption{\label{tab:opti_pose_ablation} Poses accuracy for different optimized parameters.}

\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{} l lll l lll l lll @{}}
\toprule
& \multicolumn{2}{c}{Front-Right Camera} && \multicolumn{2}{c}{LiDAR} \\
\cmidrule{2-3} \cmidrule{5-6}
Optimized parameters & Translation error (cm) & Rotation error (°) && Translation error (cm) & Rotation error (°) \\
\hline
Only spatial & $9.2\pm1.2$ & $0.44\pm0.09$ && $12.6\pm1.7$ & $0.54\pm0.08$ & \\
Only temporal & $74.8\pm0.8$\ & $8.8\pm0.05$  && $90.4\pm1.1$ & $8.8\pm0.06$ & \\
Spatial \& temporal & $2.0\pm0.4$ & $0.09\pm0.02$ && $8.9\pm3.2$ & $0.42\pm0.09$ & \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/spatial_ablation.tex <==
\begin{table*}[hbt!]
\centering
\scriptsize
\caption{\label{tab:spatial_ablation} Calibration accuracy with solely rotation or translation error.}

\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{} l l ll l ll l l @{}}
\toprule
&& \multicolumn{2}{c}{Front-Right Camera} && \multicolumn{2}{c}{LiDAR} \\
\cmidrule{3-4} \cmidrule{6-7}
Error type & Initial error & Translation error (cm) & Rotation error (°) && Translation error (cm) & Rotation error (°)  \\
\hline
\multirow{3}{*}{Rotation all axes}
& 2° & $1.6\pm0.3$ & $0.09\pm0.01$ && $9.2\pm1.9$ & $0.39\pm0.09$ \\
& 5° & $1.7\pm0.5$ & $0.07\pm0.05$ && $9.9\pm2.3$ & $0.4\pm0.14$  \\
& 10° & $127.2\pm0.6$ & $15.81\pm0.02$ && $104.4\pm1.7$ & $17.07\pm0.13$  \\ 
\hline
\multirow{3}{*}{Translation all axes}
& 20cm & $1.8\pm0.4$ & $0.09\pm0.02$ && $8.7\pm1.5$ & $0.46\pm0.1$ \\
& 50cm & $1.7\pm0.5$ & $0.09\pm0.02$ && $7.8\pm1.2$ & $0.5\pm0.06$  \\
& 100cm & $1.7\pm0.3$ & $0.09\pm0.02$ && $8.8\pm2.4$ & $0.43\pm0.08$  \\ 
\bottomrule
\end{tabular}
\end{table*}

==> tables/spatial_calibration.tex <==
\begin{table*}[hbt!]
\centering
\scriptsize
\caption{\label{tab:spatial_calibration} Spatial calibration accuracy.}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{} l l ll l ll l l @{}}
\toprule
& \multicolumn{2}{c}{Front-right camera} && \multicolumn{2}{c}{LiDAR} \\
\cmidrule{2-3} \cmidrule{5-6}
Sequence & Translation error (cm) & Rotation error (°) && Translation error (cm) & Rotation error (°) \\
\hline
0 & $2.3\pm0.6$ & $0.09\pm0.02$ && $8.2\pm1.8$ & $0.21\pm0.08$ \\
1 & $1.6\pm0.4$ & $0.09\pm0.02$ && $7.3\pm2.1$ & $0.41\pm0.08$ \\
2 & $1.2\pm0.6$ & $0.04\pm0.03$ && $13.5\pm1.8$ & $0.18\pm0.10$ \\ 
4 & $2.2\pm0.7$ & $0.08\pm0.06$ && $9.9\pm2.6$ & $0.30\pm0.10$ \\ 
\bottomrule
\end{tabular}
%\caption{caption blablabla} 
\end{table*}

==> tables/spatiotemporal_calibration.tex <==


\begin{table*}[hbt!]
\centering
\scriptsize
\caption{\label{tab:spatiotemporal_calibration} Spatiotemporal calibration accuracy.}

\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{} l cc c cc c cc c cc c cc c @{}}
\toprule
& \multicolumn{2}{c}{Rotation(°)} && \multicolumn{2}{c}{Translation(cm)}  && \multicolumn{2}{c}{Time offset(ms)} && \multicolumn{2}{c}{Training time(min)} \\ 
\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12} 
Sequence & MOISST & Our method &&  MOISST & Our method &&  MOISST & Our method &&  MOISST & Our method \\
\hline
0 & $2.1\pm1.4$ & $0.0\pm0.0$ && $41.3\pm20.3$ & $0.0\pm0$ && $4.5\pm6.0$ & $0\pm0$\\
1 & $0.3\pm0.2$ & $0.0\pm0.0$ && $20.4\pm9.7$ & $0.0\pm0$ && $4.9\pm3.5$ & $0\pm0$\\
2 & $1.3\pm1.3$ & $0.0\pm0.0$ && $47.9\pm26.1$ & $0.0\pm0$ && $5.4\pm3.9$ & $0\pm0$\\
3 & $0.6\pm0.3$ & $0.0\pm0.0$ && $28.9\pm12.7$ & $0.0\pm0$ && $15.9\pm6.7$ & $0\pm0$\\


\bottomrule
\end{tabular}
\end{table*}



==> tables/temporal_calibration.tex <==
\begin{table}[b]
\centering
\scriptsize
\caption{\label{tab:temporal_ablation} Temporal calibration accuracy.}

\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{} l l ll l ll l l @{}}
\toprule
&& Front-right camera && LiDAR \\
\cmidrule{3-3} \cmidrule{5-5}
Sequence & Initial error (ms) & Temporal error (ms) && Temporal error (ms) \\
\hline
\multirow{2}{*}{0}
& 100  & $0.7\pm0.3$ && $7.6\pm1.0$ \\
& 200  & $0.5\pm0.3$ && $6.2\pm2.0$ \\
\hline
\multirow{2}{*}{1}
& 100  & $0.2\pm0.2$ && $1.5\pm1.1$ \\
& 200  & $0.5\pm0.3$ && $1.1\pm0.5$ \\
\hline
\multirow{2}{*}{2}
& 100  & $1.0\pm0.3$ && $14.0\pm1.8$ \\
& 200  & $1.1\pm0.3$ && $13.8\pm1.2$ \\
\hline
\multirow{2}{*}{4}
& 100  & $0.6\pm0.3$ && $3.4\pm1.5$  \\
& 200  & $0.7\pm0.3$ && $14.2\pm1.5$ \\
\bottomrule
\end{tabular}
\end{table}
